NoticIA: A Clickbait Article Summarization Dataset in Spanish

We present NoticIA, a dataset consisting of 850 Spanish news articles featuring prominent clickbait headlines, each paired with high-quality, single-sentence generative summarizations written by humans. This task demands advanced text understanding and summarization abilities, challenging the models' capacity to infer and connect diverse pieces of information to meet the user's informational needs generated by the clickbait headline. We evaluate the Spanish text comprehension capabilities of a wide range of state-of-the-art large language models. Additionally, we use the dataset to train ClickbaitFighter, a task-specific model that achieves near-human performance in this task.

==> Tablas/modelsvshuman1and2.tex <==
\begin{table}[]
    \centering
    \adjustbox{max width=.9\linewidth}{
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{tabular}{@{}lcc@{}}
\toprule
                          & Rouge vs Human1 & Rouge vs Human2 \\ \midrule
gpt-4-0125-preview        & 32.25           & 28.28           \\
Nous-Hermes-2-Yi-34B      & 29.98           & 26.44           \\
openchat-3.5-0106         & 28.43           & 23.41           \\
Nous-Hermes-2-SOLAR-10.7B & 27.39           & 24.59           \\ \bottomrule
\end{tabular}}
    \caption{Rouge score of the models' predictions when computed against the summaries produced by the first and second set of annotators.}
    \label{tab:modelsvshuman1and2}
\end{table}



==> Tablas/noticia_dataset.tex <==
\begin{table}[H]
\centering
\begin{adjustbox}{width=\textwidth, totalheight=\textheight, keepaspectratio}
\begin{tabular}{lr}
\toprule
Domain Name & Count \\
\midrule
Huffingtonpost.es & 176 \\
Okdiario.com & 63 \\
Cope.es & 57 \\
Cadenaser.com & 40 \\
Mundodeportivo.com & 38 \\
Elpais.com & 24 \\
Antena3.com & 21 \\
Lecturas.com & 21 \\
Elplural.com & 16 \\
Losreplicantes.com & 15 \\
Esdiario.com & 13 \\
Ole.com & 12 \\
Lasexta.com & 11 \\
Marca.com & 11 \\
Infobae.com & 10 \\
Computerhoy.com & 10 \\
Formulatv.com & 10 \\
Adslzone.net & 9 \\
Vozpopuli.com & 9 \\
Autobild.es & 8 \\
Elespanol.com & 8 \\
Eleconomista.es & 7 \\
As.com & 7 \\
Genbeta.com & 7 \\
Semana.com & 6 \\
Eldigitaldealbacete.com & 6 \\
Sensacine.com & 6 \\
Lne.es & 6 \\
Que.es & 6 \\
Sport.es & 6 \\
Xataka.com & 6 \\
Telecinco.es & 6 \\
Elconfidencial.com & 5 \\
Eldiario.es & 5 \\
Esquire.com & 5 \\
Laopiniondemurcia.es & 5 \\
Elcorreo.com & 5 \\
Xatakandroid.com & 5 \\
Elobservador.com & 5 \\
cgixix.com & 4 \\
Foxsports.com & 4 \\
Ensedeciencia.com & 4 \\
Eldestapeweb.com & 4 \\
Espinof.com & 4 \\
Farodevigo.es & 4 \\
cnn.com & 3 \\
Hipertextual.com & 3 \\
Radioacktiva.com & 3 \\
3djuegos.com & 3 \\
Caracol.com & 3 \\
Hablandoenplata.es & 3 \\
Hibridosyelectricos.com & 3 \\
Bitlysdowssl-aws.com & 3 \\
Elconfidencialdigital.com & 3 \\
Eltiempo.com & 3 \\
Epe.es & 2 \\
Marie-claire.es & 2 \\
Tn.com & 2 \\
Elcorreoweb.es & 2 \\
Soymotor.com & 2 \\
Muyinteresante.com & 2 \\
Lavanguardia.com & 2 \\
Fotogramas.es & 2 \\
Periodistadigital.com & 2 \\
Elespectador.com & 2 \\
Nintenderos.com & 2 \\
Womenshealthmag.com & 2 \\
Rac1.cat & 2 \\
Eldesmarque.com & 2 \\
Libertaddigital.com & 2 \\
Larazon.es & 2 \\
motorsport.com & 2 \\
Elchapuzasinformatico.com & 2 \\
Publico.es & 2 \\
Informacion.es & 2 \\
Clarin.com & 2 \\
Elperiodicodearagon.com & 1 \\
Diariosanrafael.com & 1 \\
Vogue.es & 1 \\
Flooxernow.com & 1 \\
Levante-emv.com & 1 \\
Medicinaresponsable.com & 1 \\
Record.com & 1 \\
Versus.com & 1 \\
Elmundo.es & 1 \\
Elmueble.com & 1 \\
Elcomercio.es & 1 \\
Defensacentral.com & 1 \\
Somoskudasai.com & 1 \\
Heraldo.es & 1 \\
20minutos.es & 1 \\
Hobbyconsolas.com & 1 \\
Businessinsider.mx & 1 \\
Culturaocio.com & 1 \\
Bbc.com & 1 \\
Ccma.cat & 1 \\
Efe.com & 1 \\
Rtve.es & 1 \\
Los40.com & 1 \\
Deia.eus & 1 \\
3djuegos.lat & 1 \\
Eluniversal.com & 1 \\
Estadiodeportivo.com & 1 \\
Diariodesevilla.es & 1 \\
Meganoticias.cl & 1 \\
Telemadrid.es & 1 \\
Las2orillas.co & 1 \\
Elindependiente.com & 1 \\
co.uk & 1 \\
Lapaginamillonaria.com & 1 \\
Levelup.com & 1 \\
Diariouno.com & 1 \\
Eldeber.com & 1 \\
Applesfera.com & 1 \\
Cronicabalear.es & 1 \\
Lanacion.com & 1 \\
Guardianocturna.mx & 1 \\
Wradio.com & 1 \\
Atlantico.net & 1 \\
Elperiodico.com & 1 \\
Elsaltodiario.com & 1 \\
Tvazteca.com & 1 \\
Hola.com & 1 \\
Elperiodicoextremadura.com & 1 \\
Abc.com & 1 \\
Gigantes.com & 1 \\
Bekia.es & 1 \\
Tudn.com & 1 \\
Noticiasdenavarra.com & 1 \\
Noticiascaracol.com & 1 \\
Gasteizhoy.com & 1 \\
Xatakamovil.com & 1 \\
Lawebdelinformatico.es & 1 \\
Elnacional.com & 1 \\
Elnacional.cat & 1 \\
Diezminutos.es & 1 \\
Publimetro.co & 1 \\
Emisorasunidas.com & 1 \\
Nationalgeographic.com & 1 \\
Lagacetadesalamanca.es & 1 \\
Mundoxiaomi.com & 1 \\
Lavozdigital.es & 1 \\
Vidaextra.com & 1 \\
Newtral.es & 1 \\
\bottomrule
\end{tabular}
\end{adjustbox}
\caption{Top Domains by Count}
\label{table:top_domains}
\end{table}


